On Parameter Estimation in Unobserved Components Models subject to Linear Inequality Constraints

We propose a new \textit{quadratic programming-based} method of approximating a nonstandard density using a multivariate Gaussian density. Such nonstandard densities usually arise while developing posterior samplers for unobserved components models involving inequality constraints on the parameters. For instance, Chan et al. (2016) provided a new model of trend inflation with linear inequality constraints on the stochastic trend. We implemented the proposed quadratic programming-based method for this model and compared it to the existing approximation. We observed that the proposed method works as well as the existing approximation in terms of the final trend estimates while achieving gains in terms of sample efficiency.

==> sections-neurips/conclusion.tex <==
\section{Conclusion and Future Work}

We conclude that the for the sampling procedures involving approximation of a nonstandard density using a multivariate Gaussian density, the proposed quadratic programming-based approach of approximation is  useful in improving the sample efficiency. For unobserved components models involving inequality restrictions on parameters such as in \cite{chan2016bounded}, the proposed approach works as well as the existing approximation in terms of the final trend estimates while achieving greater gains in terms of sample efficiency.

We aim to implement the proposed quadratic programming-based approximation for more complex models and further improve the run-time and sample efficiency of the estimates in the future.
